ERM++: An Improved Baseline for Domain Generalization

Domain Generalization (DG) aims to develop classifiers that can generalize to new, unseen data distributions, a critical capability when collecting new domain-specific data is impractical. A common DG baseline minimizes the empirical risk on the source domains. Recent studies have shown that this approach, known as Empirical Risk Minimization (ERM), can outperform most more complex DG methods when properly tuned. However, these studies have primarily focused on a narrow set of hyperparameters, neglecting other factors that can enhance robustness and prevent overfitting and catastrophic forgetting, properties which are critical for strong DG performance. In our investigation of training data utilization (i.e., duration and setting validation splits), initialization, and additional regularizers, we find that tuning these previously overlooked factors significantly improves model generalization across diverse datasets without adding much complexity. We call this improved, yet simple baseline ERM++. Despite its ease of implementation, ERM++ improves DG performance by over 5\% compared to prior ERM baselines on a standard benchmark of 5 datasets with a ResNet-50 and over 15\% with a ViT-B/16. It also outperforms all state-of-the-art methods on DomainBed datasets with both architectures. Importantly, ERM++ is easy to integrate into existing frameworks like DomainBed, making it a practical and powerful tool for researchers and practitioners. Overall, ERM++ challenges the need for more complex DG methods by providing a stronger, more reliable baseline that maintains simplicity and ease of use. Code is available at \url{https://github.com/piotr-teterwak/erm_plusplus}

==> algo.tex <==
\begin{algorithm}[t]
\caption{\textbf{ERM++:} Components of ERM++ are annotated in the algorithm comments. We run this training loop in two passes, the first to set training length by using a validation set split from the source domains. In the second pass we train on the combination of train and val data.} \label{alg:erm++}
\begin{algorithmic}
\State $ModelWeights \gets AugmixWeights$
\Comment{Strong init}
\While{$steps \neq LongTrainSteps$}
\Comment{Long Train}
\State $X,Y \gets$ next(FullDataIterator)
\Comment{Full Data}
\If{$steps \leq 500$}
    \State Update linear classifier
 \Comment{Warmstart}
\Else
    \State Update linear classifier and backbone
\EndIf
\If{$steps \geq 600$}
\State $ModelWeightsAvg \gets $ Update  
\Comment Weight Reg.
\State $ModelWeightsAvgBN \gets $ BN stats 
\Comment UBN
\EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}


==> preamble.tex <==
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}


